Homotopy composition of cospans

It is well known that the category of finite sets and cospans, composed by pushout, contains the universal {\em special} commutative Frobenius algebra. In this note we observe that the same construction yields also general commutative Frobenius algebras, if just the pushouts are changed to homotopy pushouts.

==> bukser.tex <==

% DIMENSIONS: Every cobordism has a width of 40 and the distance
% between the centre of two input circles is 30 
% 
% The starting point is always the lower input hole, and the end
% position is always the lower output hole.  For bilinFA and cobilinFA
% the starting point is the lower hole and the end position.  couniFA 
% and unitFA leave the end position equal to the start position


% \begin{document}

% we initialise the fatness variable
\def\fatness{1.2}
\everytexdraw{%
	\drawdim pt \linewd 0.5 \textref h:C v:C
  \arrowheadsize l:4 w:3  
  \arrowheadtype t:V
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\textline}[1]{%
\phantom{(}{#1}\phantom{)}%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setbox7=\hbox{% using setbox1 doesn't work: somehow xalignat destroys it
\raisebox{1pt}{\begin{texdraw}
	\drawdim pt \linewd 0.3 \setunitscale 1.2
	\move (-3 0)
	\move (0 -1.2) 
	\rlvec (6 0) 
	\rlvec (0 -1.2)
	\rlvec (2.4 2.4) 
	\rlvec (-2.4 2.4)
	\rlvec (0 -1.2) 
	\rlvec (-6 0)
	\rlvec (0 -2.4)
	\move (11.5 0)
\end{texdraw}}}

\newcommand{\cobto}{\,\usebox7\,}


% \newcommand{\cobto}{%
% \raisebox{1pt}{\begin{texdraw}
% 	\drawdim pt \linewd 0.3 \setunitscale 1.2
% 	\move (-3 0)
% 	\move (0 -1.2) 
% 	\rlvec (6 0) 
% 	\rlvec (0 -1.2)
% 	\rlvec (2.4 2.4) 
% 	\rlvec (-2.4 2.4)
% 	\rlvec (0 -1.2) 
% 	\rlvec (-6 0)
% 	\rlvec (0 -2.4)
% 	
% 	\move (11.5 0)
% 	\end{texdraw}}
% }



\newcommand{\longcobto}{%
	\raisebox{1pt}{\begin{texdraw}
	\drawdim pt \linewd 0.3 \setunitscale 1.2
	\move (-3 0)
	\move (0 -1.2) 
	\rlvec (20 0) 
	\rlvec (0 -1.2)
	\rlvec (2.4 2.4) 
	\rlvec (-2.4 2.4)
	\rlvec (0 -1.2) 
	\rlvec (-20 0)
	\rlvec (0 -2.4)
	
	\move (25.5 0)
	\end{texdraw}}
}
\newcommand{\downcobto}{%
	\begin{texdraw}
	\drawdim pt \linewd 0.3 \setunitscale 1.2
	\move (0 6)
	
	\move (-1.2 0) 
	\rlvec (0 -12) 
	\rlvec (-1.2 0)
	\rlvec (2.4 -2.4) 
	\rlvec (2.4 2.4)
	\rlvec (-1.2 0) 
	\rlvec (0 12)
	\rlvec (-2.4 0)
	
	\move (0 -17.5)
	\end{texdraw}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\idFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 0) \lellip rx:{\xrad} ry:{\yrad}
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inB}) \rlvec (40 0) %upper edge
		\move (0 {\inA}) \rlvec (40 0) %lower edge
		\savepos (40 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\counitFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0)
		\move (20 0)
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inB}) \rlvec (8 0) %upper edge
		\move (0 {\inA}) \rlvec (8 0) %lower edge
	  \move (8 {\inA}) \clvec (20 {\inA})(20 {\inB})(8 {\inB}) %u-shape

		\savepos (0 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\unitFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0)
		\move (-20 0)
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inB}) \rlvec (-8 0) %upper edge
		\move (0 {\inA}) \rlvec (-8 0) %lower edge
	  \move (-8 {\inA}) \clvec (-20 {\inA})(-20 {\inB})(-8 {\inB}) %u-shape

		\savepos (0 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\twistFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inD}) \clvec (28 {\inD})(20 {\inB})(40 {\inB}) %upper downS
		\move (0 {\inC}) \clvec (20 {\inC})(12 {\inA})(40 {\inA}) %lower edge downS

		\move (0 {\inB}) \clvec (20 {\inB})(12 {\inD})(40 {\inD}) %upper upS
		\move (0 {\inA}) \clvec (28 {\inA})(20 {\inC})(40 {\inC}) %lower edge upS
		\savepos (40 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\twistoverFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inD}) \clvec (28 {\inD})(20 {\inB})(40 {\inB}) %upper downS
		\move (0 {\inC}) \clvec (20 {\inC})(12 {\inA})(40 {\inA}) %lower edge downS

		\move (0 {\inB}) \clvec (20 {\inB})(12 {\inD})(40 {\inD}) %upper upS
		\move (0 {\inA}) \clvec (28 {\inA})(20 {\inC})(40 {\inC}) %lower edge upS
		\savepos (40 0)(*ex *ey)
    \move (17.11 17.8) \fcir f:1 r:5
    \move (15.79 24.74) \fcir f:1 r:5
    \move (22.89 12.2) \fcir f:1 r:5
    \move (24.21 5.26) \fcir f:1 r:5
	\esegment
	\move (*ex *ey)
}
\newcommand{\twistunderFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inD}) \clvec (28 {\inD})(20 {\inB})(40 {\inB}) %upper downS
		\move (0 {\inC}) \clvec (20 {\inC})(12 {\inA})(40 {\inA}) %lower edge downS

		\move (0 {\inB}) \clvec (20 {\inB})(12 {\inD})(40 {\inD}) %upper upS
		\move (0 {\inA}) \clvec (28 {\inA})(20 {\inC})(40 {\inC}) %lower edge upS
		\savepos (40 0)(*ex *ey)
    \move (22.89 17.8) \fcir f:1 r:5
    \move (24.21 24.74) \fcir f:1 r:5

    \move (17.11 12.2) \fcir f:1 r:5
    \move (15.79 5.26) \fcir f:1 r:5
	\esegment
	\move (*ex *ey)
}
\newcommand{\multFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 15) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {15} { \yrad} \outB
		\realadd {15} {-\yrad} \outA
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
		\move (0 {\inD}) \clvec (25 {\inD})(20 {\outB})(40 {\outB}) %upper edge
		\move (0 {\inB}) \clvec (18 {\inB})(18 {\inC})(0 {\inC}) %u-shape
		\move (0 {\inA}) \clvec (25 {\inA})(20 {\outA})(40 {\outA}) %lower edge
		\savepos (40 15)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\supFA}{%
  \bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 15) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {15} { \yrad} \outB
		\realadd {15} {-\yrad} \outA
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA

		\move (0 {\inB}) \clvec (20 {\inB})(15 {\outB})(40 {\outB}) %upper edge
		\move (0 {\inA}) \clvec (25 {\inA})(20 {\outA})(40 {\outA}) %lower edge

		\savepos (40 15)(*ex *ey)
\esegment
\move (*ex *ey)
}

\newcommand{\comultFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 -15) \lellip rx:{\xrad} ry:{\yrad}
		\move (40 15) \lellip rx:{\xrad} ry:{\yrad}
		\realadd { 0} { \yrad} \outB
		\realadd { 0} {-\yrad} \outA
		\realadd {15} { \yrad} \inD
		\realadd {15} {-\yrad} \inC
		\realadd {-15} { \yrad} \inB
		\realadd {-15} {-\yrad} \inA
		\move (40 {\inD}) \clvec (15 {\inD})(20 {\outB})(0 {\outB}) %upper edge
		\move (40 {\inB}) \clvec (22 {\inB})(22 {\inC})(40 {\inC}) %u-shape
		\move (40 {\inA}) \clvec (15 {\inA})(20 {\outA})(0 {\outA}) %lower edge
		\savepos (40 -15)(*ex *ey)
	\esegment
	\move (*ex *ey)
}

\newcommand{\sdownFA}{%
   \rmove (40 -15)
  \bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (-40 15) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {15} { \yrad} \outB
		\realadd {15} {-\yrad} \outA
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA

		\move (0 {\inB}) \clvec (-20 {\inB})(-15 {\outB})(-40 {\outB}) %upper edge
		\move (0 {\inA}) \clvec (-25 {\inA})(-20 {\outA})(-40 {\outA}) %lower edge

		\savepos (0 0)(*ex *ey)
\esegment
\move (*ex *ey)
}


\newcommand{\bilinFA}{%
  \bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
				\realmult {\yrad} {2} \diam
		\realadd {24} {\diam} \storsving
		\move ({\storsving} 0) %just to get a proper bounding box

		\move (0 {\inB}) \clvec (18 {\inB})(18 {\inC})(0 {\inC}) %inner u-shape
		\move (0 {\inA}) \clvec ({\storsving} {\inA})({\storsving} {\inD})(0 {\inD}) %outer u

		
		\savepos (0 30)(*ex *ey)
\esegment
\move (*ex *ey)
}
\newcommand{\cobilinFA}{%
  \bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
				\realmult {\yrad} {2} \diam
		\realadd {24} {\diam} \storsving
		\move ({-\storsving} 0) %just to get a proper bounding box

		\move (0 {\inB}) \clvec (-18 {\inB})(-18 {\inC})(0 {\inC}) %inner u-shape
		\move (0 {\inA}) \clvec ({-\storsving} {\inA})({-\storsving} {\inD})(0 {\inD}) %outer u

		
		\savepos (0 30)(*ex *ey)
\esegment
\move (*ex *ey)
}
\newcommand{\multupFA}{%
	\bsegment
		\move (0 0) \lellip rx:3 ry:7.5
		\move (0 30) \lellip rx:3 ry:7.5
		\move (40 30) \lellip rx:3 ry:7.5
		\move (0 37.5) \clvec (15 37.5)(15 35)(22 35)\clvec (32 35)(32 37.5)(40 37.5) %upper edge
		\move (0 22.5) \clvec (20 22.5)(8 7.5)(0 7.5) %u-shape
		\move (0 -7.5) \clvec (28 -7.5)(20 22.5)(40 22.5) %lower edge
		\savepos (40 30)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\multdownFA}{%
	\bsegment
		\move (0 0) \lellip rx:3 ry:7.5
		\move (0 30) \lellip rx:3 ry:7.5
		\move (40 0) \lellip rx:3 ry:7.5
		\move (0 -7.5) \clvec (15 -7.5)(15 -5)(22 -5)\clvec (32 -5)(32 -7.5)(40 -7.5) %upper edge
		\move (0 22.5) \clvec (8 22.5)(20 7.5)(0 7.5) %u-shape
		\move (0 37.5) \clvec (28 37.5)(20 7.5)(40 7.5) %lower edge
		\savepos (40 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\comultdownFA}{%
	\bsegment
		\move (40 -30) \lellip rx:3 ry:7.5
		\move (40 0) \lellip rx:3 ry:7.5
		\move (0 0) \lellip rx:3 ry:7.5
		\move (40 7.5) \clvec (25 7.5)(25 5)(18 5)\clvec (8 5)(8 7.5)(0 7.5) %upper edge
		\move (40 -7.5) \clvec (20 -7.5)(32 -22.5)(40 -22.5) %u-shape
		\move (40 -37.5) \clvec (12 -37.5)(20 -7.5)(0 -7.5) %lower edge
		\savepos (40 -30)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\comultupFA}{%
	\bsegment
		\move (40 0) \lellip rx:3 ry:7.5
		\move (40 30) \lellip rx:3 ry:7.5
		\move (0 0) \lellip rx:3 ry:7.5
		\move (40 -7.5) \clvec (25 -7.5)(25 -5)(18 -5)\clvec (8 -5)(8 -7.5)(0 -7.5) %upper edge
		\move (40 22.5) \clvec (32 22.5)(20 7.5)(40 7.5) %u-shape
		\move (40 37.5) \clvec (12 37.5)(20 7.5)(0 7.5) %lower edge
		\savepos (40 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}

\newcommand{\sdowndownFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
% 		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (40 -30) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (40 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {0} { \yrad} \inD
		\realadd {0} {-\yrad} \inC
		\realadd {-30} { \yrad} \inB
		\realadd {-30} {-\yrad} \inA
		\move (0 {\inD}) \clvec (28 {\inD})(20 {\inB})(40 {\inB}) %upper downS
		\move (0 {\inC}) \clvec (20 {\inC})(12 {\inA})(40 {\inA}) %lower edge downS

% 		\move (0 {\inB}) \clvec (20 {\inB})(12 {\inD})(40 {\inD}) %upper upS
% 		\move (0 {\inA}) \clvec (28 {\inA})(20 {\inC})(40 {\inC}) %lower edge upS
		\savepos (40 -30)(*ex *ey)
	\esegment
	\move (*ex *ey)
}
\newcommand{\supupFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
% 		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (40 0) \lellip rx:{\xrad} ry:{\yrad}
% 		\move (40 30) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
% 		\move (0 {\inD}) \clvec (28 {\inD})(20 {\inB})(40 {\inB}) %upper downS
% 		\move (0 {\inC}) \clvec (20 {\inC})(12 {\inA})(40 {\inA}) %lower edge downS

		\move (0 {\inB}) \clvec (20 {\inB})(12 {\inD})(40 {\inD}) %upper upS
		\move (0 {\inA}) \clvec (28 {\inA})(20 {\inC})(40 {\inC}) %lower edge upS
		\savepos (40 30)(*ex *ey)
	\esegment
	\move (*ex *ey)
}



\newcommand{\threepointFA}{%
  \bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 30) \lellip rx:{\xrad} ry:{\yrad}
		\move (0 60) \lellip rx:{\xrad} ry:{\yrad}
		\realadd {60} { \yrad} \inF
		\realadd {60} {-\yrad} \inE
		\realadd {30} { \yrad} \inD
		\realadd {30} {-\yrad} \inC
		\realadd { 0} { \yrad} \inB
		\realadd { 0} {-\yrad} \inA
				\realmult {\yrad} {2} \diam
		\realadd {32} {\diam} \storsving
		\realadd {-4} {\inA} \hivA
		\realadd { 4} {\inF} \hivF
		\move ({\storsving} 0) %just to get a proper bounding box

		\move (0 {\inB}) \clvec (18 {\inB})(18 {\inC})(0 {\inC}) %inner u-shape
		\move (0 {\inD}) \clvec (18 {\inD})(18 {\inE})(0 {\inE}) %inner u-shape
		\move (0 {\inA}) \clvec ({\storsving} {\hivA})({\storsving} {\hivF})(0 {\inF}) %outer u

		
		\savepos (0 60)(*ex *ey)
\esegment
\move (*ex *ey)
}

\newcommand{\handleFA}{%
       \realmult {\fatness} {2.5} \xrad
        \realmult {\fatness} {6.25} \yrad
	\bsegment
		\rmove (40 -15)
    \bsegment
         \move (-40 15) \lellip rx:{\xrad} ry:{\yrad}
        \realadd {15} { \yrad} \outB
        \realadd {15} {-\yrad} \outA
        \realadd {30} { \yrad} \inD
        \realadd {30} {-\yrad} \inC
        \realadd { 0} { \yrad} \inB
        \realadd { 0} {-\yrad} \inA
        \move (0 {\inD}) \clvec (-25 {\inD})(-20 {\outB})(-40 {\outB}) %upper edge
        \move (0 {\inB}) \clvec (-18 {\inB})(-18 {\inC})(0 {\inC}) %u-shape
        \move (0 {\inA}) \clvec (-25 {\inA})(-20 {\outA})(-40 {\outA}) %lower edge
        \savepos (0 0)(*ex *ey)
	  \esegment
	  \move (*ex *ey)

    \bsegment
        \move (40 15) \lellip rx:{\xrad} ry:{\yrad}
        \realadd {15} { \yrad} \outB
        \realadd {15} {-\yrad} \outA
        \realadd {30} { \yrad} \inD
        \realadd {30} {-\yrad} \inC
        \realadd { 0} { \yrad} \inB
        \realadd { 0} {-\yrad} \inA
        \move (0 {\inD}) \clvec (25 {\inD})(20 {\outB})(40 {\outB}) %upper edge
        \move (0 {\inB}) \clvec (18 {\inB})(18 {\inC})(0 {\inC}) %u-shape
        \move (0 {\inA}) \clvec (25 {\inA})(20 {\outA})(40 {\outA}) %lower edge
        \savepos (40 15)(*ex *ey)
    \esegment
    \move (*ex *ey)

	\esegment
    \move (*ex *ey)
}
\newcommand{\comultmultFA}{%
\handleFA
        \realmult {\fatness} {2.5} \xrad
        \realmult {\fatness} {6.25} \yrad
        \move (40 15) \lellip rx:{\xrad} ry:{\yrad}
        \move (40 -15) \lellip rx:{\xrad} ry:{\yrad}
}

\newcommand{\tetraFA}{%
\bsegment
		\move (0 0) \lellip rx:{3} ry:{7.5}
		\move (0 30) \lellip rx:{3} ry:{7.5}
		\move (0 37.5) \clvec (25 30)(25 27.5)(40 27.5) %upper edge
              \clvec (55 27.5)(55 30)(80 37.5)
		\move (0 -7.5) \clvec (25 0)(25 2.5)(40 2.5) %lower edge
              \clvec (55 2.5)(55 0)(80 -7.5)
    \move (0 7.5) \clvec (32.5 12.5)(32.5 17.5)(0 22.5) %u-shape
    \move (80 7.5) \clvec (47.5 12.5)(47.5 17.5)(80 22.5) %u-shape
		\move (80 0) \lellip rx:{3} ry:{7.5}
		\move (80 30) \lellip rx:{3} ry:{7.5}
        \savepos (80 0)(*ex *ey)
    \esegment
    \move (*ex *ey)
}

\newcommand{\antipodeFA}{%
	\bsegment
		\move (0 0) \lellip rx:3 ry:7.5
		\move (40 0) \lellip rx:3 ry:7.5
		\move (0 7.5) \lvec (40 -7.5)
		\move (0 -7.5) \lvec (40 7.5)
		\savepos (40 0)(*ex *ey)
	\esegment
	\move (*ex *ey)
}

\newcommand{\circleFA}{%
	\bsegment
		\realmult {\fatness} {2.5} \xrad
		\realmult {\fatness} {6.25} \yrad
		\move (0 0) \lellip rx:{\xrad} ry:{\yrad}
	\esegment
}

\def\Bdot{ \fcir f:0 r:1 }
\def\BBdot{ \fcir f:0 r:2 }

\newcommand{\interval}[1]{%
  \bsegment
  \move (0 2) \lvec (0 -2)
  \move ({#1} 2) \lvec ({#1} -2)
  \move (0 0) \rlvec ({#1} 0)
  \savepos ({#1} 0)(*ex *ey)
  \esegment
  \move (*ex *ey)
}



\newcommand{\normalFA}{%
	\bsegment
    \arrowheadsize l:3 w:2
\linewd 0.3 \ravec (8 0) 
\esegment
}
\newcommand{\normalleftFA}{%
	\bsegment
  \arrowheadsize l:3 w:2
\linewd 0.3 \ravec (-8 0) 
\esegment
}
\newcommand{\normaldownFA}{%
	\bsegment
  \arrowheadsize l:3 w:2
\linewd 0.3 \ravec (0 -8) 
\esegment
}
\newcommand{\normalupFA}{%
	\bsegment
  \arrowheadsize l:3 w:2
\linewd 0.3 \ravec (0 8) 
\esegment
}


\newcommand{\intextmultFA}{%
  \raisebox{-2.2pt}{\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \multFA
  \move (-6 0)
  \move (46 0) 
  \end{texdraw}}
}
\newcommand{\intextbilinFA}{%
  \raisebox{-2.2pt}{\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \bilinFA
  \move (-6 0)
  \move (30 0) 
  \end{texdraw}}
}
\newcommand{\intextcobilinFA}{%
  \raisebox{-2.2pt}{\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \cobilinFA
  \move (6 0)
  \move (-30 0) 
  \end{texdraw}}
}
\newcommand{\intextmultcapFA}{%
  \raisebox{-2.2pt}{\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \multFA \counitFA
  \move (-6 0)
  \move (60 0) 
  \end{texdraw}}
}
\newcommand{\intextcomultFA}{%
  \raisebox{-2.3pt}{\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \comultFA
  \move (-6 0)
  \move (46 0) 
  \end{texdraw}}
}
\newcommand{\intextunitFA}{%
  \raisebox{0.9pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.45
  \unitFA
  \move (6 0)
  \end{texdraw}}
}
\newcommand{\intextcounitFA}{%
  \raisebox{0.9pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.45
  \counitFA
  \move (-6 0)
  \end{texdraw}}
}
\newcommand{\intextidFA}{%
  \raisebox{1pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.35
  \idFA
  \move (6 0)
  \end{texdraw}}
}
\newcommand{\intexthandleFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \handleFA
  \move (-6 0)
  \move (86 0)
  \end{texdraw}}
}
\newcommand{\intextcomultmultFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \handleFA
  \move (-6 0)
  \move (86 0)
  \end{texdraw}}
}
\newcommand{\intextmultcomultFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \multFA\comultFA
  \move (-6 0)
  \move (86 0)
  \end{texdraw}}
}

\newcommand{\intexttwocylFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \idFA
  \move (0 30) \idFA
  \move (-6 0)
  \move (46 0)
  \end{texdraw}}
}

\newcommand{\intexttwistFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \twistFA \move (46 0) \move (-6 0)
  \end{texdraw}}
}
\newcommand{\intexttwisttwistFA}{%
  \raisebox{-2.3pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.3
  \twistFA \twistFA  \move (86 0) \move (-6 0)
  \end{texdraw}}
}

\newcommand{\intextantipodeFA}{%
  \raisebox{1pt}
  {\begin{texdraw}
  \drawdim pt \linewd 0.3 \setunitscale 0.35
  \antipodeFA
  \move (6 0)
  \end{texdraw}}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                %
%   RELATIONS AND OTHER CHUNKS   %
%                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\assRelFA}{% eventually the second part should be hard coded too!
\move (0 -30) \bsegment
		\move (0 0) \lellip rx:3 ry:7.5
		\move (0 30) \lellip rx:3 ry:7.5
		\move (0 60) \lellip rx:3 ry:7.5
		\move (40 15) \lellip rx:3 ry:7.5
		\move (40 45) \lellip rx:3 ry:7.5
		\move (80 30) \lellip rx:3 ry:7.5
	
		\move (0 67.5) \clvec (25 67.5)(20 52.5)(40 52.5)
                   \clvec (65 52.5)(60 37.5)(80 37.5) %upper edge
		\move (0 -7.5) \clvec (25 -7.5)(20 7.5)(40 7.5)
                   \clvec (65 7.5)(60 22.5)(80 22.5) %lower edge
		\move (0 52.5) \clvec (20 52.5)(15 37.5)(40 37.5)
		               \clvec (58 37.5)(58 22.5)(40 22.5)
	                 \clvec (20 22.5)(25 37.5)(0 37.5) %upper bay (long)
		\move (0 7.5) \clvec (18 7.5)(18 22.5)(0 22.5) %lower bay
\esegment
		\htext (105 0){$=$}
	\move (130 -30)\bsegment
		\move (0 0) \lellip rx:3 ry:7.5
		\move (0 30) \lellip rx:3 ry:7.5
		\move (0 60) \lellip rx:3 ry:7.5
		\move (40 15) \lellip rx:3 ry:7.5
		\move (40 45) \lellip rx:3 ry:7.5
		\move (80 30) \lellip rx:3 ry:7.5
	
		\move (0 67.5) \clvec (25 67.5)(20 52.5)(40 52.5)
                   \clvec (65 52.5)(60 37.5)(80 37.5) %upper edge
		\move (0 -7.5) \clvec (25 -7.5)(20 7.5)(40 7.5)
                   \clvec (65 7.5)(60 22.5)(80 22.5) %lower edge
		\move (0 7.5) \clvec (20 7.5)(15 22.5)(40 22.5)
		               \clvec (58 22.5)(58 37.5)(40 37.5)
	                 \clvec (20 37.5)(25 22.5)(0 22.5) %lower bay (long)
		\move (0 52.5) \clvec (18 52.5)(18 37.5)(0 37.5) %upper bay
\esegment
\move (210 0)
}
\newcommand{\coassRelFA}{% eventually this should be hard coded!
	\move (0 0)
	\comultFA
	\comultFA
	\rmove (-40 45)
	\supFA
		\htext (105 0){$=$}
	\move (130 0)
	\comultFA
	\sdownFA
	\rmove (-40 45)
	\comultFA
}

\newcommand{\commRelFA}{% eventually this should be hard coded!
	\move (0 -15)
	\twistFA
	\multFA
		\htext (105 0){$=$}
	\move (130 -15)
	\multFA
}
\newcommand{\cocommRelFA}{% eventually this should be hard coded!
	\move (0 0)
	\comultFA
	\twistFA
		\htext (105 0){$=$}
	\move (130 0)
	\comultFA
}

\newcommand{\unitRelFA}{% eventually this should be hard coded!
	\move (40 -15)
	\unitFA
	\multFA
  \move (0 15) \idFA
		\htext (100 0){$=$}
	\move (120 0)
	\idFA
		\htext (180 0){$=$}
		\move (200 -15)
    \bsegment
	\idFA \multFA
  \move (40 30)	\unitFA
	\esegment
}
\newcommand{\counitRelFA}{% eventually this should be hard coded!
	\bsegment
	\comultFA
  \idFA
  \rmove (-40 30) \counitFA
  \esegment
		\htext (100 0){$=$}
	\move (120 0)
	\idFA
		\htext (180 0){$=$}
		\move (200 0)
    \bsegment
	\comultFA \counitFA
  \move (40 15)	\idFA
	\esegment
}
\newcommand{\SFA}{% hard coded edges
	\bsegment
		\move ( 0  0) \lellip rx:3 ry:7.5
		\move ( 0 30) \lellip rx:3 ry:7.5
		\move (40 45) \lellip rx:3 ry:7.5
		\move (40 15) \lellip rx:3 ry:7.5
		\move (40 -15) \lellip rx:3 ry:7.5
		\move (80  0) \lellip rx:3 ry:7.5
		\move (80 30) \lellip rx:3 ry:7.5

    \move (0 37.5) \clvec (20 37.5)(15 52.5)(40 52.5)
                   \clvec (65 52.5)(60 37.5)(80 37.5) %upper edge
    \move (0 -7.5) \clvec (20 -7.5)(15 -22.5)(40 -22.5)
                   \clvec (65 -22.5)(60 -7.5)(80 -7.5) %lower edge
		\move (80 22.5) \clvec (55 22.5)(60 37.5)(40 37.5)
                    \clvec (22 37.5)(22 22.5)(40 22.5)
                    \clvec (65 22.5)(60 7.5)(80 7.5) %upper-right bay
		\move (0 7.5) \clvec (25 7.5)(20 -7.5)(40 -7.5)
                    \clvec (58 -7.5)(58 7.5)(40 7.5)
                    \clvec (15 7.5)(20 22.5)(0 22.5) %lower-left bay
		\savepos (80 0)(*ex *ey)
	\esegment
  \move (*ex *ey)
}
\newcommand{\ZFA}{% hard coded edges
	\bsegment
		\move ( 0  0) \lellip rx:3 ry:7.5
		\move ( 0 30) \lellip rx:3 ry:7.5
		\move (40 45) \lellip rx:3 ry:7.5
		\move (40 15) \lellip rx:3 ry:7.5
		\move (40 -15) \lellip rx:3 ry:7.5
		\move (80  0) \lellip rx:3 ry:7.5
		\move (80 30) \lellip rx:3 ry:7.5

    \move (0 37.5) \clvec (20 37.5)(15 52.5)(40 52.5)
                   \clvec (65 52.5)(60 37.5)(80 37.5) %upper edge
    \move (0 -7.5) \clvec (20 -7.5)(15 -22.5)(40 -22.5)
                   \clvec (65 -22.5)(60 -7.5)(80 -7.5) %lower edge
		\move (0 22.5) \clvec (25 22.5)(20 37.5)(40 37.5)
                    \clvec (58 37.5)(58 22.5)(40 22.5)
                    \clvec (15 22.5)(20 7.5)(0 7.5) %upper-left bay
		\move (80 7.5) \clvec (55 7.5)(60 -7.5)(40 -7.5)
                    \clvec (22 -7.5)(22 7.5)(40 7.5)
                    \clvec (65 7.5)(60 22.5)(80 22.5) %lower-right bay
		\savepos (80 0)(*ex *ey)
	\esegment
  \move (*ex *ey)
}

\newcommand{\frobRelFA}{% hard coded via SFA and ZFA
  \SFA
  \htext (110 15){$=$}
  \move (140 0)
  \multFA \comultFA
  \htext (250 15){$=$}
  \move (280 0)
  \ZFA
}

\newcommand{\snakeRelFA}{%
			\move (0 0)
			\bsegment
			\idFA
			\bilinFA
			\cobilinFA
			\idFA
			\esegment
							\htext (105 30){$=$}

			\move (130 30)
			\bsegment
			\idFA
			\esegment
							\htext (195 30){$=$}

			\move (260 0)
			\bsegment
			\idFA
			\rmove (-40 0)
			\cobilinFA
			\bilinFA
			\rmove (-40 0)
			\idFA
			\esegment
}

\newcommand{\greydiscOP}[1]{%
  \bsegment
    \fcir f:0.8 r:{#1} \lcir r:{#1} 
    \bsegment \linewd 0.3 \arrowheadsize l:3 w:2 \move ({#1} 0) \ravec (5 0) \esegment
  \esegment
}
\newcommand{\whitediscOP}[1]{%
  \bsegment
    \fcir f:1 r:{#1} \lcir r:{#1} 
    \bsegment \linewd 0.3 \arrowheadsize l:3 w:2 \move ({#1} 0) \ravec (5 0) \esegment
  \esegment
}
\newcommand{\circleOP}[1]{%
  \bsegment
    \lcir r:{#1} 
    \bsegment \linewd 0.3 \arrowheadsize l:3 w:2 \move ({#1} 0) \ravec (5 0) \esegment
  \esegment
}






\newcommand{\onedot}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\esegment
}
\newcommand{\twodots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}
\newcommand{\threedots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}
\newcommand{\fourdots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}
\newcommand{\fivedots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}
\newcommand{\sixdots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}
\newcommand{\sevendots}[1]{
  \bsegment
	\move (0 0) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\rmove (0 {#1}) \fcir f:0 r:2
	\esegment
}



\newcommand{\strand}[2]{%
	\bsegment
		\realmult {#1} {.5} \halfway
		\move (0 0) \clvec ({\halfway} 0)({\halfway} {#2})({#1} {#2})
		\savepos ({#1} {#2})(*ex *ey)
	\esegment
	\move (*ex *ey)
}

